Particle creation in the presence of a warped extra dimension

Particle creation in spacetimes with a warped extra dimension is studied. In particular, we investigate the dynamics of a conformally coupled, massless scalar field in a five dimensional warped geometry where the induced metric on the 3--branes is that of a spatially flat cosmological model. We look at situations where the scale of the extra dimension is assumed (i) to be time independent or (ii) to have specific functional forms for time dependence. The warp factor is chosen to be that of the Randall--Sundrum model. With particular choices for the functional form of the scale factor (and also the function characterising the time evolution of the extra dimension) we obtain the ${| \beta_k|}^2$, the particle number and energy densities after solving (wherever possible, analytically but, otherwise, numerically) the conformal scalar field equations. The behaviour of these quantities for the massless and massive Kaluza--Klein modes are examined. Our results show the effect of a warped extra dimension on particle creation and illustrate how the nature of particle production on the brane depends on the nature of warping, type of cosmological evolution as well as the temporal evolution of the extra dimension.

==> fitplots.tex <==
\begin{figure}[!ht]
\includegraphics[width=4in,height=6.5in,angle=-90]{thermalfit.eps}
\caption{Best-fit plots by a thermal radiation for datapoints of $k^2|\beta_k|^2$ vs. $k$ (top-left plot in right box of Fig.\ref{fig:PN&peqAn} where $b_1 = 0.2$$, b_2 = 1$, for 3 values of $k_\sigma$, such as $2.17463$(upper curve), $5.00365$(middle curve) and $8.03846$(lower curve)), and the corresponding best-fitting parameter values.} \label{fig:thermalfit} 
\end{figure}
\begin{figure}[!ht]
\includegraphics[width=4in,height=6.5in,angle=-90]{nonthermalfit.eps}
\caption{Best-fit plots by a nonthermal radiation for datapoints of $k^2|\beta_k|^2$ vs. $k$ (top-left plot in right box of Fig.\ref{fig:PN&peqAn} where $b_1 = 0.2$$, b_2 = 1$, for 3 values of $k_\sigma$, such as $2.17463$(upper curve), $5.00365$(middle curve) and $8.03846$(lower curve)), and the corresponding best-fitting parameter values.} \label{fig:nonthermalfit} 
\end{figure}


==> list_of_changes <==

List of changes
---------------

1. In response to the query of the referee regarding the use of the
index `l' to represent `k' and `k_\sigma' in Eqn 2.16 and subsequently,
integrate over `l' in Eqns 2.19, 2.20, we have made the following change.

The integrations in 2.19 are, actually over `k', at fixed `k_\sigma'--
this is shown explicitly now. The `l' index in \beta_l remains
because \beta_l depends on both k and k_\sigma, though, we eventually
calculate the number and energy densities at fixed k_\sigma values.

2. We have added several references now. These appear as [12], [16],[17],
[18] and [20]  and are appropriately cited in the text.

3. An `Acknowledgments' section has been added.


